From Hybrid Modal Logic to Matching Logic and Back

Building on our previous work on hybrid polyadic modal logic we identify modal logic equivalents for Matching Logic, a logic for program specification and verification. This provides a rigorous way to transfer results between the two approaches, which should benefit both systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{M. Marin, A. Cr\u{a}ciun (Eds.): \\
Working Formal Methods Symposium 2019 (FROM 2019)\\
EPTCS 303, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.303.2}{10.4204/EPTCS.303.2}}
\pdfoutput=1

